Direct and spillover effects of a new tramway line on the commercial vitality of peripheral streets. A synthetic-control approach

In cities, the creation of public transport infrastructure such as light rails can cause changes on a very detailed spatial scale, with different stories unfolding next to each other within a same urban neighborhood. We study the direct effect of a light rail line built in Florence (Italy) on the retail density of the street where it was built and and its spillover effect on other streets in the treated street's neighborhood. To this aim, we investigate the use of the Synthetic Control Group (SCG) methods in panel comparative case studies where interference between the treated and the untreated units is plausible, an issue still little researched in the SCG methodological literature. We frame our discussion in the potential outcomes approach. Under a partial interference assumption, we formally define relevant direct and spillover causal effects. We also consider the ``unrealized'' spillover effect on the treated street in the hypothetical scenario that another street in the treated unit's neighborhood had been assigned to the intervention.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
